Global Public Sentiment on Decentralized Finance: A Spatiotemporal Analysis of Geo-tagged Tweets from 150 Countries

Blockchain technology and decentralized finance (DeFi) are reshaping global financial systems. Despite their impact, the spatial distribution of public sentiment and its economic and geopolitical determinants are often overlooked. This study analyzes over 150 million geo-tagged, DeFi-related tweets from 2012 to 2022, sourced from a larger dataset of 7.4 billion tweets. Using sentiment scores from a BERT-based multilingual classification model, we integrated these tweets with economic and geopolitical data to create a multimodal dataset. Employing techniques like sentiment analysis, spatial econometrics, clustering, and topic modeling, we uncovered significant global variations in DeFi engagement and sentiment. Our findings indicate that economic development significantly influences DeFi engagement, particularly after 2015. Geographically weighted regression analysis revealed GDP per capita as a key predictor of DeFi tweet proportions, with its impact growing following major increases in cryptocurrency values such as bitcoin. While wealthier nations are more actively engaged in DeFi discourse, the lowest-income countries often discuss DeFi in terms of financial security and sudden wealth. Conversely, middle-income countries relate DeFi to social and religious themes, whereas high-income countries view it mainly as a speculative instrument or entertainment. This research advances interdisciplinary studies in computational social science and finance and supports open science by making our dataset and code available on GitHub, and providing a non-code workflow on the KNIME platform. These contributions enable a broad range of scholars to explore DeFi adoption and sentiment, aiding policymakers, regulators, and developers in promoting financial inclusion and responsible DeFi engagement globally.

==> tables/dictionary/dictionary_archive.tex <==
\renewcommand{\arraystretch}{3}
\setlength{\tabcolsep}{1pt}
\begin{table}[H]
\centering
\begin{adjustbox}{max width=1.3\textwidth}
{\large
\begin{tabular}{|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{2.5cm}|L{3cm}|}
\hline
English Keywords    & Chinese (Simplified) Keywords & Chinese (Traditional)   Keywords & Japanese       & Korean Keywords & Russian Keywords & German Keywords  & French Keywords  & Spanish Keywords  & Italian Keywords & Portuguese   Keywords & Arabic Keywords    & Hindi Keywords         & Dutch Keywords   & Swedish Keywords & Danish Keywords  & Polish Keywords  & Turkish Keywords & Greek Keywords   & Finnish Keywords & Norwegian   Keywords & Tags          \\
\hline
blockchain          & 区块链                          & 區塊鏈                             & ブロックチェーン       & 블록체인            & блокчейн         & blockchain       & chaîne de blocs  & cadena de bloques & blockchain       & blockchain            & سلسلة الكتل        & ब्लॉकचेन               & blockchain       & blockkedja       & blockchain       & łańcuch bloków   & blok zinciri     & μπλοκτσέιν       & lohkoketju       & \multicolumn{2}{|l|}{blockchain}       \\
\hline
NFT                 & 非同质化代币                       & 非同質化代幣                          & 非代替性トークン       & 비대체 토큰          & НФТ              & NFT              & NFT              & NFT               & NFT              & NFT                   & NFT                & NFT                    & NFT              & NFT              & NFT              & NFT              & NFT              & NFT              & NFT              & NFT                  &               \\
\hline
crypto              & 加密货币                         & 加密貨幣                            & 暗号通貨           & 암호화폐            & крипто           & crypto           & crypto           & crypto            & crypto           & crypto                & كريبتو             & क्रिप्टोमुद्रा         & crypto           & crypto           & crypto           & crypto           & crypto           & crypto           & crypto           & crypto               &               \\
\hline
Bitcoin             & 比特币                          & 比特幣                             & ビットコイン         & 비트코인            & биткоин          & Bitcoin          & Bitcoin          & Bitcoin           & Bitcoin          & Bitcoin               & بيتكوين            & बिटकॉइन                & Bitcoin          & Bitcoin          & Bitcoin          & Bitcoin          & Bitcoin          & Bitcoin          & Bitcoin          & Bitcoin              & \#BTC,\$BTC   \\
\hline
Ethereum            & 以太坊                          & 以太坊                             & イーサリアム         & 이더리움            & Эфириум          & Ethereum         & Ethereum         & Ethereum          & Ethereum         & Ethereum              & إثريوم             & इथेरियम                & Ethereum         & Ethereum         & Ethereum         & Ethereum         & Ethereum         & Ethereum         & Ethereum         & Ethereum             & \$ETH         \\
\hline
Binance             & 币安                           & 幣安                              & バイナンス          & 바이낸스            & Бинанс           & Binance          & Binance          & Binance           & Binance          & Binance               & بينانس             & बिनेंस                 & Binance          & Binance          & Binance          & Binance          & Binance          & Binance          & Binance          & Binance              & \#BNB,\$BNB   \\
\hline
Dogecoin            & 狗狗币                          & 狗狗幣                             & ドージコイン         & 도지코인            & догекоин         & Dogecoin         & Dogecoin         & Dogecoin          & Dogecoin         & Dogecoin              & دوجكوين            & डोगेकोइन               & Dogecoin         & Dogecoin         & Dogecoin         & Dogecoin         & Dogecoin         & Dogecoin         & Dogecoin         & Dogecoin             & \#DOGE,\$DOGE \\
\hline
Ripple              & 瑞波                           & 瑞波                              & リップル           & 리플              & Риппл            & Ripple           & Ripple           & Ripple            & Ripple           & Ripple                & ريبل               & रिप्पल                 & Ripple           & Ripple           & Ripple           & Ripple           & Ripple           & Ripple           & Ripple           & Ripple               & \#XRP,\$XRP   \\
\hline
Litecoin            & 莱特币                          & 萊特幣                             & ライトコイン         & 라이트코인           & Лайткоин         & Litecoin         & Litecoin         & Litecoin          & Litecoin         & Litecoin              & لايتكوين           & लाइटकॉइन               & Litecoin         & Litecoin         & Litecoin         & Litecoin         & Litecoin         & Litecoin         & Litecoin         & Litecoin             & \#LTC,\$LTC   \\
\hline
USD Coin,   USDCoin & USD币|USDC币                   & USD幣|USDC幣                      & USDコイン|USDCコイン & USD코인|USDC코인    & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin  & USD Coin|USDCoin & USD Coin|USDCoin      & عملة USD|عملة USDC & USD मुद्रा|USDC मुद्रा & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin & USD Coin|USDCoin     & \#USDC,\$USDC \\
\hline
Tether              & 泰达币                          & 泰達幣                             & テザーコイン         & USDT            & USDT             & Tether           & Tether           & Tether            & Tether           & Tether                & USDT               & USDT                   & Tether           & Tether           & Tether           & Tether           & Tether           & Tether           & Tether           & Tether               & \#USDT,\$USDT \\
\hline
Cardano             & 卡尔达诺                         & 卡爾達諾                            & カルダノ           & 카르다노            & Кардано          & Cardano          & Cardano          & Cardano           & Cardano          & Cardano               & كاردانو            & कार्डानो               & Cardano          & Cardano          & Cardano          & Cardano          & Cardano          & Cardano          & Cardano          & Cardano              & \#ADA,\$ADA   \\
\hline
Solana              & 索拉纳                          & 索拉納                             & ソラナ            & 솔라나             & Solana           & Solana           & Solana           & Solana            & Solana           & Solana                & سولانا             & Solana                 & Solana           & Solana           & Solana           & Solana           & Solana           & Solana           & Solana           & Solana               & \#SOL,\$SOL   \\
\hline
\#TRON              & 波场币                          & 波場幣                             & \#TRON         & \#TRON          & \#TRON           & \#TRON           & \#TRON           & \#TRON            & \#TRON           & \#TRON                & \#TRON             & \#TRON                 & \#TRON           & \#TRON           & \#TRON           & \#TRON           & \#TRON           & \#TRON           & \#TRON           & \#TRON               & \#TRX,\$TRX  \\ \hline
\end{tabular}
}
\end{adjustbox}
\end{table}


==> tables/spatial/autocorrelation_archive.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\begin{table*}%[H]
\centering
\caption{Spatial autocorrelation}
\label{tab:autocorrelation}
\begin{tblr}{
  width = \linewidth,
  colspec = {|Q[200]|Q[170]|Q[150]|Q[150]|Q[150]|Q[150]|Q[150]|},
  row{1} = {c},
  column{4} = {c},
  column{5} = {c},
  column{6} = {c},
  column{7} = {c},
  cell{1}{3} = {c},
  cell{2}{3} = {c},
  cell{3}{3} = {c},
  cell{4}{3} = {c},
  cell{5}{3} = {c},
  cell{6}{3} = {c},
  cell{7}{3} = {c},
  cell{8}{3} = {c},
  cell{9}{3} = {c},
  hline{1,3-10} = {-}{},
  hline{2} = {3-7}{},
}
Variable & Test & Weights &  &  &  & \\
 &  & 1-nearest neighbor & 2-nearest neighbor & 3-nearest neighbor & 4-nearest neighbor & 5-nearest neighbor\\
ln(GDP per capita) & Moran's I & 0.800*** (0.100) & 0.751*** (0.075) & 0.704*** (0.061) & 0.687*** (0.054) & 0.675*** (0.047)\\
ln(Tweet proportion) & Moran's I & 0.357*** (0.101) & 0.368*** (0.074) & 0.358*** (0.061) & 0.340*** (0.053) & 0.328*** (0.047)\\
Sentiment score & Moran's I & 0.282** (0.100) & 0.162* (0.073) & 0.151** (0.059) & 0.156** (0.051) & 0.160*** (0.047)\\
 &  &  &  &  &  & \\
Cluster 1 (binary) & Chi-square & 4.700* & 7.298** & 10.980*** & 12.285*** & 12.159***\\
Cluster 2 (binary) & Chi-square & 5.686* & 15.614*** & 19.548*** & 25.459*** & 27.293***\\
Cluster 3 (binary) & Chi-square & 22.697*** & 38.920*** & 46.047*** & 66.707*** & 72.755***
\end{tblr}

\raggedright
\small \textit{Note}: This table presents the results of the spatial autocorrelation analysis using Moran’s I and Chi-square tests across different spatial weight structures. 

- \textbf{Moran’s I for GDP per capita, tweet proportion, and sentiment score}: The positive and statistically significant Moran’s I values indicate strong spatial clustering, meaning that similar values of these variables tend to be geographically concentrated. The effect is strongest for GDP per capita, suggesting that wealthier countries tend to cluster together. The spatial autocorrelation for tweet proportion and sentiment score, while weaker, remains significant across different nearest-neighbor specifications.

- \textbf{Chi-square tests for country clusters}: The spatial distribution of country clusters is tested using Chi-square statistics. Higher values indicate stronger clustering patterns. Cluster 3 (high-GDP countries) exhibits the highest level of spatial clustering, followed by Cluster 2 and then Cluster 1. This suggests that economic and social factors influencing decentralized finance discussions are not randomly distributed but form distinct spatial patterns.

- \textbf{Nearest-neighbor approach}: The table reports results using 1 to 5 nearest neighbors to define spatial relationships. The decreasing magnitude of Moran’s I values as more distant neighbors are included suggests that spatial autocorrelation weakens with distance.

- \textbf{Statistical significance levels}: $p$ $<$ 0.05 (*), $p$ $<$ 0.01 (**), and $p$ $<$ 0.001 (***) indicate the robustness of these spatial effects.
These findings emphasize that economic and social characteristics influencing decentralized finance discussions exhibit strong spatial dependencies. This reinforces the need for geographically weighted models when analyzing these trends.

\end{table*}
